Learning Color Compatibility in Fashion Outfits

Color compatibility is important for evaluating the compatibility of a fashion outfit, yet it was neglected in previous studies. We bring this important problem to researchers' attention and present a compatibility learning framework as solution to various fashion tasks. The framework consists of a novel way to model outfit compatibility and an innovative learning scheme. Specifically, we model the outfits as graphs and propose a novel graph construction to better utilize the power of graph neural networks. Then we utilize both ground-truth labels and pseudo labels to train the compatibility model in a weakly-supervised manner.Extensive experimental results verify the importance of color compatibility alone with the effectiveness of our framework. With color information alone, our model's performance is already comparable to previous methods that use deep image features. Our full model combining the aforementioned contributions set the new state-of-the-art in fashion compatibility prediction.

==> figure_TSNE.tex <==
\begin{figure}
\centering
\includegraphics[trim=50 40 50 40, clip,width=\linewidth]{figures/i1864t_cluster.pdf}
\caption{TSNE visualization of the outfit embeddings obtained from a model trained with one negative cluster. The black points are the samples whose compatibility are wrongly predicted and the points in other colors are the samples whose compatibility are correctly predicted. Furthermore, each color indicates a different cluster predicted by the trained model.}
\label{fig:TSNE}
\end{figure}

==> figure_color_palettes.tex <==
\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Examples of fashion images and our extracted color palettes}
\label{fig:color_palettes}
\end{figure}

==> figure_global_local.tex <==
\begin{figure}
\centering
\includegraphics[trim=0 0 520 0, clip,width=\linewidth]{figures/global_local.pdf}
\caption{Graph constructions for global and local supervision of a given pair of samples. For global supervision, all items in the outfits are used. For local supervision, common items in the positive-negative sample pair are not used. Eliminated nodes and edges are denoted in dotted lines.}
\label{fig:global_local}
\end{figure}

==> figure_recommendation.tex <==
\begin{figure}
\begin{center}
\begin{subfigure}[b]{0.4\linewidth}
	\centering
	\includegraphics[trim=0 314 440 0, clip,width=\linewidth]{figures/recommendation_13.pdf}
	\caption{Cluster 1 v.s. Cluster 3}
	\label{fig:recommendation2}
\end{subfigure}
\hspace{5pt}
\begin{subfigure}[b]{0.4\linewidth}
	\centering
	\includegraphics[trim=0 314 440 0, clip,width=\linewidth]{figures/recommendation_14.pdf}
	\caption{Cluster 1 v.s. Cluster 4}
	\label{fig:recommendation1}
\end{subfigure}
\begin{subfigure}[b]{0.4\linewidth}
	\centering
	\includegraphics[trim=0 314 440 0, clip,width=\linewidth]{figures/recommendation_23.pdf}
	\caption{Cluster 2 v.s. Cluster 3}
	\label{fig:recommendation3}
\end{subfigure}
\hspace{5pt}
\begin{subfigure}[b]{0.4\linewidth}
	\centering
	\includegraphics[trim=0 314 440 0, clip,width=\linewidth]{figures/recommendation_24.pdf}
	\caption{Cluster 2 v.s. Cluster 4}
	\label{fig:recommendation4}
\end{subfigure}
\end{center}
   \caption{For each subplot, Left: fashion items of the given incomplete outfits. Right: fashion item recommendation based on different patterns of compatible colors.}
\label{fig:recommendation}
\end{figure}

==> figure_sample_color.tex <==
\begin{figure*}
\begin{center}
\begin{subfigure}[b]{\linewidth}
	\centering
	\includegraphics[trim=0 400 110 0, clip,width=0.9\linewidth]{figures/LabO3_cluster1_eg.pdf}
	\caption{Cluster 1: The visualization suggests that the items of the outfits in this cluster have similar colors.}
	\label{fig:sample1}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
	\centering
	\includegraphics[trim=0 400 110 0, clip,width=0.9\linewidth]{figures/LabO3_cluster2_eg.pdf}
	\caption{Cluster 2: The visualization suggests that the outfits in this cluster have the combination of two major colors that distinct in hues but similar in chromas and lightnesses, and one neutral color.}
	\label{fig:sample2}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
	\centering
	\includegraphics[trim=0 400 110 0, clip,width=0.9\linewidth]{figures/LabO3_cluster3_eg.pdf}
	\caption{Cluster 3: The visualization suggests that the items of the outfits in this cluster have colors in high variance of hues, chromas and lightnesses.}
	\label{fig:sample3}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
	\centering
	\includegraphics[trim=0 400 110 0, clip,width=0.9\linewidth]{figures/LabO3_cluster4_eg.pdf}
	\caption{Cluster 4: The visualization suggests that the outfits in this cluster have colors in high contrast of chromas. Specifically, there are one major color with high chroma as spotlight and one neutral color (black, white) for balance.}
	\label{fig:sample4}
\end{subfigure}
\end{center}
   \caption{Compatible outfit clusters predicted using color palettes as fashion representation. Due to limited space, we only display 50 outfits per cluster and at most 10 items per outfit in a column. Two outfit samples in the bounding boxes are enlarged and shown on the right.}
\label{fig:sample_color}
\end{figure*}

==> figure_supp_cluster.tex <==
\begin{figure*}
\centering
\includegraphics[trim=0 270 200 0, clip,width=\linewidth]{figures/supp_cluster.pdf}
\caption{Examples of outfits in each predicted cluster. The experiments were conducted on the testing set of the Polyvore Outfits dataset using the proposed method with color palettes. Each outfit is displayed in a row.}
\label{fig:supp_cluster}
\end{figure*}

==> figure_supp_sample_it.tex <==
\begin{figure*}
\begin{center}
\begin{subfigure}[b]{\linewidth}
	\centering
	\includegraphics[trim=0 0 0 0, clip,width=\linewidth]{figures/i1864t_sample_cluster5_12_50.jpg}
	\caption{This cluster reveals two mixed color patterns. One pattern consists of similar colors, whereas the other pattern shows contrast colors.}
	\label{fig:supp_sample_it1}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
	\centering
	\includegraphics[trim=0 0 0 0, clip,width=\linewidth]{figures/i1864t_sample_cluster6_12_50.jpg}
	\caption{This cluster contains multiple color patterns that are hard to interpret directly.}
	\label{fig:supp_sample_it2}
\end{subfigure}
\end{center}
   \caption{Compatible outfit clusters predicted using color palettes as fashion representation. Due to limited space, we only display 50 outfits per cluster. The 50 outfits are shown on the left where items in the same column belong to the same outfit.}
\label{fig:supp_sample_it}
\end{figure*}

==> table_cluster.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
\#clusters & 
Compat AUC & FITB Acc\\
\hhline{|=|=|=|}
3 & 0.84 & 54.2\\ 
5 & 0.84 & 58.8 \\
7 & 0.84 & 56.9 \\
9 & 0.84 & 55.1\\
\hline
\end{tabular}
\end{center}
\caption{Effect of different choices of cluster numbers. The experiments are conducted on the validation set of Polyvore Outfits with color palettes as fashion representations.}
\label{tb:cluster}
\end{table}


==> table_lambda.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
$\lambda$ & 
Compat AUC & FITB Acc\\
\hhline{|=|=|=|}
0 & 0.84 & 54.7\\ 
0.5 & 0.84 & 58.8 \\
1 & 0.84 &  57.1\\
5 & 0.83 & 50.5\\
\hline
\end{tabular}
\end{center}
\caption{Effect of different choices of $\lambda$. The experiments are conducted on the validation set of Polyvore Outfits with color palettes as fashion representations.}
\label{tb:lambda}
\end{table}


==> table_main_results.tex <==
\begin{table*}[!t]
%\begin{center}
\caption{Comparison with previous methods in different settings.} 
\label{tb:main}
\begin{subtable}[b]{\linewidth}
\begin{center}
\caption{Comparison with previous methods using color palettes or deep image features.}
\label{tb:img_results}
\begin{tabular}{|p{2.6cm}|p{2cm}|c|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|}
\hline
\multirow{2}{2.6cm}{Methods}  & \multirow{2}{2cm}{Image representation} & \multirow{2}{1.2cm}{Needs category}
& \multicolumn{2}{|c|}{P. Outfits} & \multicolumn{2}{|c|}{Maryland P.} \\
\cline{4-7}
& & & CP & FITB & CP & FITB \\
\hhline{|=|=|=|=|=|=|=|}
%
Siamese Net\cite{[2015ICCV]Learning} & ResNet18 & - &0.81 & 52.9 & 0.85 & 54.4\\
\hline
Type-aware\cite{[2018ECCV]Learning} & ResNet18 & Yes & 0.83 & 54.0 & 0.87 & 57.9\\
\hline
Outfit gen.\cite{[2019arxiv]Coherent} & ResNet18 & - &
0.90 & 59.1 & 0.89 & 59.8 \\
\hline
Context-aware\cite{[2019CVPR]Context} & ResNet50 & - &
--- & --- & 0.76 & 47.0 \\
\hline
NGNN\cite{[2019WWW]Dressing} & ResNet18 & Yes & 
0.78 & 53.0 & 0.66 & 37.2\\
\hline
CSA-Net\cite{[2020CVPR]Fashion} & ResNet18 & Yes &
\textbf{0.91} & \textbf{63.7} & --- & ---\\
\hline
\multirow{2}{2.6cm}{Ours} & Color palette & - & 
0.84 & 58.0 & 0.83 & 49.1\\
& ResNet18 & - &
\textbf{0.91} & 59.2 & \textbf{0.91} & \textbf{59.9}\\
\hline
\end{tabular}
\end{center}
\end{subtable}

\begin{subtable}[b]{\linewidth}
\begin{center}
\caption{Comparison with previous methods when text information is additionally utilized.}
\label{tb:img_text_results}
\begin{tabular}{|p{2.05cm}|p{3.15cm}|c|c|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|}
\hline
\multirow{2}{2.05cm}{Methods} & \multirow{2}{3.15cm}{Image / text representation} & \multirow{2}{1.2cm}{Needs category} 
& \multirow{2}{1.55cm}{Needs text in testing}
& \multicolumn{2}{|c|}{P. Outfits} & \multicolumn{2}{|c|}{Maryland P.} \\
\cline{5-8}
& & & & CP & FITB & CP & FITB \\
\hhline{|=|=|=|=|=|=|=|=|}
Bi-LSTM\cite{[2017MM]Learning} & InceptionV3/HGLMM & Yes & - &
0.65 & 39.7 & \textbf{0.94} & 64.9\\
\hline
Type-aware\cite{[2018ECCV]Learning} & ResNet18/HGLMM & Yes & - & 
0.86 & 55.3 & 0.90 & 61.0\\
\hline
Outfit gen.\cite{[2019arxiv]Coherent} & ResNet18/BERT & - & Yes &
\textbf{0.93} & \textbf{66.1} & 0.93 & \textbf{69.9}\\
\hline
SCE-Net\cite{[2019ICCV]Learning} & ResNet18/HGLMM & - & Yes &
0.91 & 61.6 & 0.90 & 60.8\\
\hline
Ours & ResNet18/HGLMM & - & - & 
0.90 & 65.8 & 0.91 & 67.1\\
\hline
\end{tabular}
\end{center}
\end{subtable}
%\end{center}
\end{table*}

